A Bregman-Sinkhorn Algorithm for the Maximum Weight Independent Set Problem

We propose a scalable approximate algorithm for the NP-hard maximum-weight independent set problem, based on dual coordinate descent applied to a smoothed clique-cover LP relaxation. Our method, a variant of the Bregman/Sinkhorn algorithm, employs entropy smoothing with a novel duality-gap-based smoothing scheduling strategy that empirically outperforms standard feasibility scheduling for the relaxed problem. Our new projection to the primal feasible set enables accurate duality gap estimation. Combined with a basic primal heuristic leveraging reduced costs, our approach yields high-quality integer solutions. On real-world datasets, it efficiently finds high-quality approximate solutions for graphs with up to 882,000 nodes and 344 million edges within seconds.

==> floats/primal-heuristic.tex <==
\begin{algorithm}[t]
  \addtolength{\hsize}{1.5em}%
  \DontPrintSemicolon
  \KwIn{$\vc\in \BR^{n}$, $\vx\in\{0,1\}^{n+m}$ feasible for~\eqref{equ:clique-relaxation}} \tcc{Input: reduced costs and feasible solution}
  \While{stopping criterion not fulfilled}{
    \tcc{generate a feasible solution:}
    $\SC' \coloneq \emptyset$\;
    \While{$\SC'\neq [m]$}{
      \tcc{randomly generate a clique from $[m]\backslash\SC'$:}
      $j \coloneq \text{random}([m]\backslash\SC')$\;
      \tcc{set locally best variable to 1:}
      $i^*\in\argmax_{i\in K_j} c_i\,; \quad x_{i^*} \coloneq 1$\;
      \tcc{... and conflicting variables to 0:}
      \For{$j'\in J_i$}{
        $x_{i} \coloneq 0$,\ $\forall i\in K_{j'}\backslash\{i^*\}$\;
        $\SC' \coloneq \SC'\cup K_{j'}$ \tcc{cliques $K_{j'}$ are done}
      }
    }
    \tcc{recombine with a current solution}
  }
  \caption{Primal heuristic}
  \label{alg:primal-heuristic}
\end{algorithm}


==> floats/table-metamis-generated-cliques.tex <==
\begin{table}
    \footnotesize
    \newcommand\rot[1]{\rotatebox{90}{#1}}
    \newcommand\Header[1]{\multicolumn{1}{c}{#1}}
    \newcommand\HeaderSeconds{t,~sec}
    \centerline{%
      \begin{tabular}{lc rrrr rrrr}
        \toprule
        && \multicolumn{2}{c}{Our (3,600 sec)}
        & \multicolumn{2}{c}{``Cold'' (\cf \cite[Tab.\,2]{dong2025metaheuristic})}
        & \multicolumn{3}{c}{``Warm'' (\cf \cite[Tab.\,3]{dong2025metaheuristic})}
        \\
        \cmidrule(r){3-4} \cmidrule(lr){5-6} \cmidrule(l){7-9}
        &&& time in \emph{s} until & \multicolumn{2}{c}{time in \emph{s} to surpass \ldots} & \multicolumn{3}{c}{time in \emph{s} to surpass \ldots}
        \\
        \Header{Dataset}
        & \Header{Instance}
        & \Header{Objective}
        & \Header{LP-Gap 0.1\,\%}
        & \Header{ILSVND}
        & \Header{METAMIS}
        & \Header{ILSVND}
        & \Header{METAMIS}
        & \Header{METAMIS+LP}
        \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % BEGIN AUTO GENERATED
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \multirow{17}{*}{\rot{AVR-LARGE}}
         & CR-S-L-1 & \textbf{5,646,433} & 260 & 6 & 73 & 728 & --- & --- \\
         & CR-S-L-2 & \textbf{5,736,183} & 259 & 10 & 174 & 811 & --- & --- \\
         & CR-S-L-4 & \textbf{5,731,512} & 265 & 9 & 127 & 995 & --- & --- \\
         & CR-S-L-6 & \textbf{3,915,519} & 94 & 5 & 28 & 750 & --- & --- \\
         & CR-S-L-7 & \textbf{2,011,518} & 11 & 2 & 12 & 524 & --- & --- \\
         & CR-T-C-1 & \textbf{4,717,956} & 39 & 2 & 13 & 163 & --- & --- \\
         & CR-T-C-2 & \textbf{4,942,913} & 109 & 2 & 22 & 240 & --- & --- \\
         & CR-T-D-4 & \textbf{4,881,499} & 180 & 3 & 29 & 767 & --- & --- \\
         & CR-T-D-6 & \textbf{3,012,364} & 71 & 1 & 8 & 380 & --- & --- \\
         & CR-T-D-7 & \textbf{1,454,429} & 9 & $<$ 1 & 3 & --- & --- & --- \\
         & CW-S-L-1 & \textbf{1,647,937} & 136 & 17 & 95 & --- & --- & --- \\
         & CW-S-L-2 & \textbf{1,723,454} & 160 & 16 & 109 & --- & --- & --- \\
         & CW-S-L-4 & \textbf{1,732,816} & 101 & 34 & 550 & --- & --- & --- \\
         & CW-S-L-6 & \textbf{1,165,691} & 30 & 17 & 102 & --- & --- & --- \\
         & CW-S-L-7 & \textbf{590,005} & 7 & 9 & 263 & --- & --- & --- \\
         & CW-T-C-1 & \textbf{1,326,021} & 13 & 8 & 134 & --- & --- & --- \\
         & CW-T-C-2 & \textbf{936,741} & 8 & 12 & 130 & --- & --- & --- \\
        \midrule
        \multirow{16}{*}{\rot{AVR-MEDIUM}}
         & CW-T-D-4 & \textbf{460,010} & 2 & $<$ 1 & 3 & 16 & --- & --- \\
         & CW-T-D-6 & \textbf{459,909} & 2 & 2 & 29 & 238 & --- & --- \\
         & MR-D-03 & \textbf{1,757,878,476} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & 5 & 39 \\
         & MR-D-05 & \textbf{1,790,072,991} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & 1 & 6 \\
         & MR-D-FN & \textbf{1,802,369,969} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & 1 & 4 \\
         & MR-W-FN & \textbf{5,386,842,781} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 \\
         & MT-D-200 & \textbf{287,155,108} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 \\
         & MT-D-FN & 290,800,404 & $<$ 1 & $<$ 1 & --- & $<$ 1 & $<$ 1 & $<$ 1 \\
         & MT-W-200 & \textbf{384,056,012} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 \\
         & MT-W-FN & \textbf{390,869,891} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 \\
         & MW-D-20 & \textbf{526,931,511} & $<$ 1 & $<$ 1 & 1 & $<$ 1 & 2 & 4 \\
         & MW-D-40 & \textbf{538,769,213} & $<$ 1 & $<$ 1 & 2 & $<$ 1 & 1 & 2 \\
         & MW-D-FN & \textbf{545,432,177} & $<$ 1 & $<$ 1 & 2 & 2 & 7 & 18 \\
         & MW-W-05 & \textbf{1,329,638,653} & 19 & 1,907 & 1,907 & 1,907 & 1,907 & 1,907 \\
         & MW-W-10 & 1,278,217,690 & 21 & --- & --- & --- & --- & --- \\
         & MW-W-FN & 1,248,966,779 & 24 & --- & --- & --- & --- & --- \\
        \midrule
        \multirow{5}{*}{\rot{AVR-SMALL}}
         & MR-D-01 & \textbf{1,691,267,110} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 \\
         & MT-D-01 & \textit{238,166,485} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 \\
         & MT-W-01 & \textit{312,121,568} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 \\
         & MW-D-01 & 476,301,619 & $<$ 1 & 1 & --- & $<$ 1 & 1 & 1 \\
         & MW-W-01 & \textit{1,270,305,952} & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 & $<$ 1 \\
        \midrule
        \multirow{3}{*}{\rot{ALL}}
         & & \multicolumn{2}{l}{\tiny\bfseries better objective: 31} \\
         & & \multicolumn{2}{l}{\tiny\itshape equal objective:    3} \\
         & & \multicolumn{2}{l}{\tiny         worse objective:    4} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % END AUTO GENERATED
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \bottomrule
      \end{tabular}}

  \caption{
    \textbf{Comparison of \cref{alg:exp-domain-stabilized} with our primal heuristic, duality gap scheduling and heuristic truncation denoted as \emph{Our} to METAMIS~\citep{dong2025metaheuristic} and ILSVND~\citep{nogueira2018hybrid} based on \citet[Tab.\,4-7]{dong2025metaheuristic}.}
    All algorithms have been run for 3,600 seconds.
    Datasets are sorted by their size, from the largest on top to the smallest in the bottom.
    \textbf{``Warm''} and \textbf{``Cold''} columns correspond to competing algorithms that use or, respectively, do not use a warm-start with a specific (not used by \emph{Our}) initial solution as explained in \citet{dong2025metaheuristic}.
    %
    \textbf{LP-Gap 0.1\%} -- time required to attain the 0.1\% relative duality gap for the relaxed problem. \textbf{ILSVND, METAMIS, METAMIS+LP} -- time required by \emph{Our} algorithm to attain the best value of the respective competing method. This value is taken from the column ``w'' in \citet[Tab.\,4-7]{dong2025metaheuristic}.
    To obtain the full time of \emph{Our} algorithm its time should be added to the respective value in the ``LP-Gap 0.1\,\%'' column. Objective value marked as \textbf{bold} means that this is \emph{strictly greater} than those obtained by any competing algorithm with the ``Cold''-start. \emph{Italic} font means that our value and value of the best competing algorithm coincide: For two of them, MT-D-01 and MT-W-01, this value furthermore coincides with the LP bound and is, therefore, optimal.
    Although \emph{Our} method only uses a comparably simple primal heuristics, it outperforms its competitors due to the usage of the reduced costs, see a detailed explanation in the main text.
  }
  \label{tab:metamis-comparison-appendix}
\end{table}

